Gaming the Game: Honeypot Venues Against Cheaters in Location-based Social Networks

The proliferation of location-based social networks (LBSNs) has provided the community with an abundant source of information that can be exploited and used in many different ways. LBSNs offer a number of conveniences to its participants, such as - but not limited to - a list of places in the vicinity of a user, recommendations for an area never explored before provided by other peers, tracking of friends, monetary rewards in the form of special deals from the venues visited as well as a cheap way of advertisement for the latter. However, service convenience and security have followed disjoint paths in LBSNs and users can misuse the offered features. The major threat for the service providers is that of fake check-ins. Users can easily manipulate the localization module of the underlying application and declare their presence in a counterfeit location. The incentives for these behaviors can be both earning monetary as well as virtual rewards. Therefore, while fake check-ins driven from the former motive can cause monetary losses, those aiming in virtual rewards are also harmful. In particular, they can significantly degrade the services offered from the LBSN providers (such as recommendations) or third parties using these data (e.g., urban planners). In this paper, we propose and analyze a honeypot venue-based solution, enhanced with a challenge-response scheme, that flags users who are generating fake spatial information. We believe that our work will stimulate further research on this important topic and will provide new directions with regards to possible solutions.

==> importance.tex <==
\section{The effects of fake check-ins}
\label{sec:importance}

Traditionally, social information systems and information quality have followed disjoint paths.
However, the presence of low quality of information (QoI) results in a decreased value for the specific platform.  
For instance, a very representative type of social information systems, vulnerable to low QoI is the Q\&A social networks \cite{zhang07} \cite{kpele-collaboratecom}.  
In these systems, people post questions that can be answered from their peers, and are focused on providing an efficient platform for enabling the crowdsourcing nature of the underlying system.  
However, no care is taken for the actual quality of the answers provided.  
In the case of Q\&A networks, feedback from users can be roughly used as a metric of the quality of the answer provided.   

While similar issues exist related to the location sharing in LBSNs, there are no systems to date that are able to filter fake check-ins to a great extent.    
However, the existence of forged spatial information in the network can have significant effects in a wide spectrum of the underlying functionalities.  
In this section we will discuss two representative examples; 
one related to the effects on participating businesses and one related to the services possibly offered by the LBSN provider.

%\subsection{Monetary Losses}

{\bf Monetary Losses: }
LBSNs have recently evolved into an {\em inexpensive} marketing channel for local businesses.  
Users can obtain special offers by checking-in at participating venues. 
This gives the latter an opportunity to be advertised, in an inexpensive way, only to people that actually have the potential to visit them.  
A traditional advertisement, which targets the majority of the population is expensive because of the volume of its target mass.  
However, only a percentage of the people exposed to it can actually benefit from the advertised good/service (e.g., people that are spatially located nearby).      

Special deals lead to a temporary loss for the locale offering it.  
This is especially true for one-time deals, such as the ones offered in Groupon \cite{byers12}.  
The rational behind these offers is that people visiting the venue will come back and hence, this will make up for the temporary loss.  
Hence, participating venues in LBSN offers might require more than one visit in an attempt to minimize the associated loss.  
For instance, Figure \ref{fig:special} provides an example of a special offer, which requires 3 check-ins.  
If the cost of the offer is $c$ (in our example $c=\$5$), the locale's gain would be reduced by $c$ for every visit if the deal was offered to every check-in.  
By requiring three check-ins the gain is only reduced by $\dfrac{c}{3}$ for every visit.   

\begin{figure}[h]
\centering \includegraphics[scale=0.8]{figures/loyalty.pdf}
\vspace{-0.1in}
\caption{An example of a special offer requiring 3 check-ins.}
\label{fig:special}
\vspace{-0.1in}
\end{figure}


Jack who wants to unlock this offer but does not want to have to go three times to the venue and spend on average $s - \dfrac{c}{3}$ per visit, where $s$ is the average expenditure of a client in the locale, can game the system and create two initial fake check-ins.  
This will enable him be present in the locale only once and unlock the deal.  
His expenditure will be only $s-c$, and the venue owner will have a reduced gain (the cost of the offer will again be $c$ per visit).  
Assuming that $s=\$20$ in our example, the locale's gain is reduced by $\$5$/client instead of the $\dfrac{5}{3}=\$1.6$/client that was the target, while the cost per visit for Jack is reduced to $\$15$ instead of $20-\dfrac{5}{3} = \$18.4$.  
Hence, it is evident that there can be monetary losses for businesses that want to use LBSNs as an  advertisement channel.  
A detection system should be developed in order to filter forged check-ins and establish a secure way for venues offering deals.  
If the latter is not in place, business owners will have a reduced incentive to participate in similar systems.  

%\subsection{Degraded Services} 
{\bf Degraded Services: }
Recently, Foursquare - the largest LBSN to date - launched a novel recommendation engine, which considers check-ins from all users in order to provide recommendations \cite{fsq-recommendation} \cite{fsq-redesign}.  
This engine takes into account user's check-ins, friend's check-ins, venue's check-ins and many other factors in order to provide suggestions.  
It should be evident that {\em noisy} data will not yield high quality service.  
Therefore, not only should LBSNs filter fake check-ins that can harm businesses (as aforementioned), but also identify any kind of fake check-ins (e.g., from gamers that simply want to gain as many virtual rewards as possible by checking-in to venues they have never been).  
Unless only ``True'' data are used from the LBSN provider to provide services, the latter will be degraded and of low quality.  

Hence, it is evident that fake check-in detection is crucial to the long-run success of the LBSN paradigm.  
In the following section, we present our initial efforts on this problem. 
  
%This noisy data can either be due to users creating multiple fake check-ins to venues for obtaining specials as aforementioned, or due to users that are intrested into the gaming aspects of the systems and check-in to places they have never been in order to gain virtual rewards.    
   
